RGB-Phase Speckle: Cross-Scene Stereo 3D Reconstruction via Wrapped Pre-Normalization

3D reconstruction garners increasing attention alongside the advancement of high-level image applications, where dense stereo matching (DSM) serves as a pivotal technique. Previous studies often rely on publicly available datasets for training, focusing on modifying network architectures or incorporating specialized modules to extract domain-invariant features and thus improve model robustness. In contrast, inspired by single-frame structured-light phase-shifting encoding, this study introduces RGB-Speckle, a cross-scene 3D reconstruction framework based on an active stereo camera system, designed to enhance robustness. Specifically, we propose a novel phase pre-normalization encoding-decoding method: first, we randomly perturb phase-shift maps and embed them into the three RGB channels to generate color speckle patterns; subsequently, the camera captures phase-encoded images modulated by objects as input to a stereo matching network. This technique effectively mitigates external interference and ensures consistent input data for RGB-Speckle, thereby bolstering cross-domain 3D reconstruction stability. To validate the proposed method, we conduct complex experiments: (1) construct a color speckle dataset for complex scenarios based on the proposed encoding scheme; (2) evaluate the impact of the phase pre-normalization encoding-decoding technique on 3D reconstruction accuracy; and (3) further investigate its robustness across diverse conditions. Experimental results demonstrate that the proposed RGB-Speckle model offers significant advantages in cross-domain and cross-scene 3D reconstruction tasks, enhancing model generalization and reinforcing robustness in challenging environments, thus providing a novel solution for robust 3D reconstruction research.

==> sec_final/0_abstract.tex <==
\begin{abstract}
    3D reconstruction garners increasing attention alongside the advancement of high-level image applications, where dense stereo matching (DSM) serves as a pivotal technique. Previous studies often rely on publicly available datasets for training, focusing on modifying network architectures or incorporating specialized modules to extract domain-invariant features and thus improve model robustness. In contrast, inspired by single-frame structured-light phase-shifting encoding, this study introduces RGB-Speckle, a cross-scene 3D reconstruction framework based on an active stereo camera system, designed to enhance robustness. Specifically, we propose a novel phase pre-normalization encoding-decoding method: first, we randomly perturb phase-shift maps and embed them into the three RGB channels to generate color speckle patterns; subsequently, the camera captures phase-encoded images modulated by objects as input to a stereo matching network. This technique effectively mitigates external interference and ensures consistent input data for RGB-Speckle, thereby bolstering cross-domain 3D reconstruction stability. To validate the proposed method, we conduct complex experiments: (1) construct a color speckle dataset for complex scenarios based on the proposed encoding scheme; (2) evaluate the impact of the phase pre-normalization encoding-decoding technique on 3D reconstruction accuracy; and (3) further investigate its robustness across diverse conditions. Experimental results demonstrate that the proposed RGB-Speckle model offers significant advantages in cross-domain and cross-scene 3D reconstruction tasks, enhancing model generalization and reinforcing robustness in challenging environments, thus providing a novel solution for robust 3D reconstruction research.
\end{abstract}

==> sec_final/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

3D reconstruction involves extracting geometric information from images of the measured object. This technique finds extensive application across diverse fields, including industrial inspection, biomedical imaging, Simultaneous Localization and Mapping (SLAM) navigation, and optical image measurement\cite{LU2022106873,ZHU2023107542,VANCROMBRUGGE2020106305,VANDERJEUGHT201618}, owing to its non-contact sensing, rapidity, and high precision. The effectiveness of these advantages largely depends on the speed and robustness of the reconstruction algorithm employed. In this regard, 3D perception schemes primarily based on multi-frame structured light and binocular vision routes have emerged as popular approaches, inspired further advancements. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/fig1_showboard.png}
    \caption{Comparison of the performance in challenging scenes. Columns from left to right denote sample input RGB image,the predicted disparities of the with rgb-speckle datasets,input phase image, the predicted disparities of the IGEV trained with phase pre-normalized images on the same datasets.}
    \label{fig:intro}
\end{figure}

However, the multi-frame projection method is restricted in scenarios involving motion or limited image capture time due to interference from vibrations and motion between image capture intervals. Single-frame methods represented by Fourier Transform Profilometry (FTP)\cite{Liu2021HighDR,LIU2019217} and Moire Technique (MT)\cite{Li:17,CHEN2023109666,Ordones:21}  do not rely on multi-frame projection. At the same time, both of them are sensitive to noise and suffer from spectrum aliasing and leakage when reconstructing objects with strong textures or steep surfaces\cite{XIAO201719,Wang:21,Wang:20}. The single-frame fringe projection 3D measurement method can use machine learning for wrapped phase prediction and phase-shifted fringe prediction. Convolutional neural networks combined with fringe analysis achieve high-precision results in a laboratory environment. These networks are supervised and trained using a large number of simulated or real stripe images and high-precision ground truth. Variants of networks such as FCN\cite{DBLP:journals/corr/LongSD14}, AEN\cite{DBLP:journals/corr/abs-1902-09314}, and U-Net\cite{DBLP:journals/corr/RonnebergerFB15} have been studied as backbone of end-to-end networks, with U-Net being the most popular\cite{Wan:23}. However, the "one-shot" method which captures only one frame of image cannot obtain robust scene information under complex lighting conditions\cite{BURNES2022106788,ODOWD2020106293}. This causes accuracy reduction of 3D reconstruction, especially in dynamic scenes or extremely short exposure conditions.

Binocular vision inherits the advantages of single-frame 3D measurement. With the release of the Scene Flow dataset, DispNet \cite{Mayer_2016} has achieved a breakthrough in the stereo matching field using an encoder-decoder structure. Networks based on the encoder-decoder structure have been developed, as examples of PSMNet \cite{chang2018pyramid} and BGNet \cite{xu2021bilateral}. The stereo matching network based on 3DCNN replicates the classic stereo matching process, including cost calculation and cost aggregation \cite{Wang_2021,shen2022pcwnet,wang2020improving}. Combining classic multi-view geometry and deep learning has repeatedly achieved state-of-the-art results \cite{10203487,chabra2019stereodrnet}. However, 4D cost volume filtering is computationally intensive and consumes enormous memory, making it difficult to generalize to images with millions of pixels \cite{duggal2019deeppruner,xu2020aanet}. Recently, iterative optimization-based methods have been proven to simplify the cost aggregation operation. Yet some inherent problems still need to be addressed: creating typical stereo datasets is labor-intensive and expensive, often limiting the scene scope \cite{Zhao2022EAIStereoEA,tosi2021smdnets,wang2021scvstereo,xu2023iterative,Wang_2024_CVPR}. Trained models perform well in a limited set of scenarios, but without fine-tuning, they perform disappointingly on cross-scenario tasks \cite{zhang2020domain,tonioni2019learning,pang2018zoom}. 

The application of state-of-the-art (SOTA) stereo matching networks to measurements remains an intractable problem. This challenge is further exacerbated when dealing with out-of-domain, low-quality, or perturbed samples. Inspired by phase truncation in structured light techniques, we propose a novel approach that combines Phase Measuring Profilometry \cite{Zheng:17,LI2022106990,Li:16,SONG201674} with stereo matching networks, introducing a color phase speckle projection. By utilizing the PMP-encoded phase speckle map instead of RGB \cite{WU2022107955,KEMAO2022106874} texture as the input for the model, our method enables consistent calculations across various scenes. This approach empowers the model to learn matching relationships and pattern similarities, effectively mitigating obstacles arising from environmental illumination changes and texture discrepancies. When the reflectivity of the object surface changes drastically and the lighting conditions are more stringent, higher requirements are placed on the generalization of the proposed method for reconstruction in the scene. There are many common problems in real scenes, such as environmental color cast, occlusion, uneven reflectance and texture interference. There are many obstacles in the cross-scene reconstruction of the previous stereo matching model using real data sets, which makes it difficult to extend to unseen scenes. As shown in Figure \ref{fig:intro}, our method can achieve better cross-scene reconstruction performance in contrast.

The contributions of this work are summarized as follows:
\begin{itemize}
\item We designed a novel encoding approach by randomly perturbing the phase shift map and integrating it into the three RGB channels to generate a color speckle pattern, which is then projected onto the scene to incorporate prior information.

\item A phase pre-normalization method is proposed to mitigate the interference from environmental lighting and texture while ensuring domain consistency among different input image pairs before entering the stereo matching network. This approach enables stereo matching network trained with this method to exhibit superior reconstruction performance in scenes projected with RGB speckle patterns containing phase information, even for unseen scenes.

\item we constructed a large RGB speckle realistic datasets with sub-pixel precision, capturing realistic and challenging scenes using an active binocular system. We conducted quantitative and qualitative experiments based on this foundation, and the results show that experiments performed on both public datasets and this speckle dataset confirm the robustness and generalizability of our approach.

\end{itemize}

==> sec_final/2_relatedwork.tex <==
\section{Related Work}
\label{sec:related}


\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.85\textwidth]{images/fig2_pipeline.png} 
    \caption{The pipeline of our method. By projecting phase-encoded color speckle patterns onto the scene during image capture and applying phase pre-normalization, robust reconstruction can be achieved across different scenes using a stereo matching network trained on speckle dataset.}
    \label{fig:pipeline}
    \end{figure*}

\paragraph{Structured light 3D reconstruction}
is considered one of the premier methodologies for optical 3D measurement. In principle, it involves projecting one or several patterns onto the surface of the target \cite{KEMAO2022106874,Feng:15,LU2022106873} and then establishing correspondences between the projector and the camera using these projected motifs. By leveraging the triangulation principle, it becomes feasible to reconstruct the three-dimensional scene through the integration of calibration data with phase unwrapping techniques \cite{Wang:17}. Of them, Fringe Projection Profilometry (FPP) is renowned for its reliability in profiling surfaces \cite{WU2022107004,YU2022128236}, but there are significant obstacles in extracting accurate and steadfast absolute phase information from a single fringe image poses substantial hurdles, limiting its efficacy in dynamic 3D reconstructions \cite{article03}. Speckle Projection Profilometry (SPP) facilitates the establishment of correspondences across stereo images by projecting a singular speckle pattern \cite{article01,Su2019TheoreticalAO}, thus enabling single-shot 3D reconstructions. However, most research primarily focuses on encoding positional data and deciphering correspondences, often overlooking a crucial aspect - minimizing interference caused by ambient light and implicit attributes inherent in the captured image \cite{article02}. 

\paragraph{Stereo matching}
 estimates a pixel-to-pixel map between two frames of images, and typically comprises four main steps: cost computation, cost aggregation, disparity calculation, and disparity refinement\cite{wu2019semantic,zhang2019ganet,tankovich2023hitnet}. In real-world uncertainty conditions (i.e., conditions affected by occlusion, smoothness, reflections, and noise), estimating disparity poses a challenging task\cite{taniai2017continuous,9337529}. With the profound transformation brought by deep learning to computer vision, convolutional neural networks (CNNs) have been introduced into stereo matching pipelines\cite{pang2018cascade,7299044,Seki2016PatchBC}. By exploring different feature representations and aggregation algorithms for matching costs, CNNs can address these challenges\cite{7780983}. For example, Mayer et al. proposed an end-to-end network for estimating disparities  and optical flows  \cite{dosovitskiy2015flownet}, along with a synthetic dataset called Scene Flow, which has become widely used for stereo tasks. In 2017, kenda firstly combined 3DCNN with the classic stereo matching pipeline for cost aggregation\cite{kendall2017endtoend}. Guo et al. proposed a more efficient group-wise correlation volume computation method, capable of better measuring the feature correlation between the left and right images \cite{guo2019groupwise}. Shen et al. adopted a cascade cost volume and adjusted the disparity search range adaptively in subsequent processes based on variance uncertainty estimation  \cite{shen2021cfnet}. Xu et al. obtained attention weights from correlation features to suppress redundant information in the concatenated volume and enhance its expressive capability \cite{xu2022attention}. Chen et al.optimize feature channels through motif channel projection instead of direct network optimization to mitigate imbalanced nonlinear transformations in network training\cite{Chen_2024_CVPR}. Gong et al. learn intra-view geometric and cross-view knowledge for stereo matching networks from an interest point detector and an an interest point matcher\cite{Gong_2024_CVPR}. End-to-end network structures dominated by 3D CNNs exhibit satisfactory performance and even produce high-quality results in pathological areas on ideal disparity maps of public datasets\cite{7410474,du2019amnet,song2021adastereo}. Although these models performed well in the training phase on specific datasets, their ability to generalize to natural scenes has not been validated. Moreover, the model heavily relies on a large amount of high-quality ground truth, it remains unexplored how to make the binocular matching model perform good results on unseen datasets.

It is the focus of cross-domain stereo matching research to be unaffected by pre-offset between different data sets. In this regard, Zhang et al. proposed a new domain normalization method, which normalizes the distribution of learning representations and makes them invariant to domain differences\cite{zhang2020domain}. Chuah W Q et al. proposed an information theory shortcut avoidance method, the information related to the shortcut is automatically limited to be encoded into the feature representation\cite{chuah2022itsa}. Pang et al. proposed a semi-supervised method using scale information\cite{pang2018zoom}. Guo et al. proposed a cross-domain method using knowledge extraction\cite{guo2018learning}. Recently, Zhang et al. avoided domain generalization ability degraded from synthetic to real by dividing pixels into consistent and inconsistent regions based on the difference between ground truth and pseudo label\cite{zhang2024robust}. However, these methods do not implement standard and complete domain adaptation channels, and their adaptation performance is very limited. Differert from these methods, we propose a robust RGB-Phase Speckle method based on pseudo-random arrays, which improve the generalizability of the algorithm by making it insensitive to ambient lighting using phase feature constraints.

Different from these methods, by introducing additional prior information and normalizing the scene, our approach bypasses the challenges of cross-domain generalization faced by stereo matching networks. It ensures domain consistency across input data, thereby preventing the network from overfitting to domain-specific datasets during training.



==> sec_final/3_proposed.tex <==
\section{Proposed Method}

This section outlines the methodological architecture of the RGB-Phase Speckle approach. Starting with presenting the RGB-Phase Speckle formula, we introduce the underlying principles that bolster its efficacy directly from the formulation. Then, we introduced the color speckle dataset under complex scenes produced according to the proposed method, which can be used for training stereo matching networks under cross-scene applications. The pipeline of our method is shown in Figure \ref{fig:pipeline}.

\subsection{RGB-Phase Speckle}

The phase information can reflect the height change of the surface of the object. Inspired by color phase-shifted fringe patterns based on phase measuring profilometry\cite{LIU2020106267}, our patterns are composed from three phase-shifted speckles encoded in the RGB channels.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/fig3_speckle.png}
    \caption{The generation process of phase color speckle pattern is disturbed and upsampled in the same way on a phase-shifting fringe and merged into three RGB channels to realize the phase-shifting coding of a single image.}
    \label{fig:rgb}
\end{figure}

To mitigate the impact of an object's inherent texture on color fringe information, we apply identical scrambling to the three-step phase-shifting fringes to generate the color speckle pattern. This approach ensures that the phase modulation at each point on the object remains independent of the relative positional relationships between the fringes, thereby facilitating network training. Furthermore, upsampling from a low-resolution speckle image prevents the speckle pattern from being submerged in sensor noise. The speckle generation process is illustrated in Figure\ref{fig:rgb}.

Taking the red channel pattern in the projector as an example, \((x^p,y^p)\) represents the pixel coordinates of the projected pattern, \(a^p\) denotes the background intensity, and \(b^p\) represents the amplitude,  \(\varphi^p(x^p,y^p)\) represents the encoded phase, \(G^p\left(x^p, y^p\right)\) is the superposition of the phase-related pattern. The RGB channels have a phase difference of \( \frac{2\pi}{3} \) to each other. The combined colors of the blue channel \(B^p(x^p, y^p)\), green channel \(G^p(x^p, y^p)\), and red channel \(G^p(x^p, y^p)\) are as follows:
\begin{align}
    B^p\left(x^p, y^p\right)=a^p+b^p \cos \left[\varphi^p(x^p,y^p) - \frac{2\pi}{3} \right]
\end{align}
\begin{align}
    G^p\left(x^p, y^p\right)=a^p+b^p \cos \left[\varphi^p(x^p,y^p)\right]
\end{align}
\begin{align}
    R^p\left(x^p, y^p\right)=a^p+b^p \cos \left[ \varphi^p(x^p,y^p) +\frac{2\pi}{3} \right]
\end{align}

It is noteworthy that the single CMOS color camera employ a Bayer array color filter placed in front of the sensor with a demosaicing algorithm used to interpolate the RGB values of pixels. Due to manufacturing imperfections, the passband ranges of the color filters for different channels partially overlap. Light reflections at wavelengths within these overlapping regions induce crosstalk among pixels across different channels, resulting in shifts in interpolation-estimated pixel values and introducing a phase deviation, denoted as $\Delta\varphi$. This deviation constitutes a non-negligible error in structured light systems relying on single-camera projection. In binocular systems, where the phase deviation $\Delta\varphi$ is consistent across both cameras, our projection pattern has no adverse effect on stereo matching performance. Thus, our approach requires no strict consistency in the projected color speckle patterns, such as eliminating the need for precise three-channel alignment.
%值得注意的是，目前单CMOS的彩色相机都是通过在图像传感器前，放置一层bayer阵列彩色滤光片，并且使用demosacing算法插值得到像素的RGB值，而由于制造工艺等影响，不同颜色的滤光片通带范围存在部分重叠，重叠区域波长的光反射进入相机的不同通道像的元后会形成串扰，再插值估计的像素值变化导致相位偏移，这对于单相机的投影的结构光系统来说是不可忽视的误差，然而，双目立体匹配中，由于左右相机中的相位偏移是一致的，因此我们的投影图案不会对匹配造成负面影响。所以我们的方法对于投影彩色散斑图案的一致性也没有要求，不同散斑图的随机打乱方式无需严格一致甚至三个通道无需严格对齐，

\subsection{Phase Pre-Normalization}

Our RGB phase speckle patterns introduce prior information into the scene. However, this phase information is embedded within the color speckle texture projected onto the object. Variations in reflectance and illumination conditions across objects in different scenes, coupled with inconsistencies in the image signal processing (ISP) algorithms of different cameras, result in domain shifts in the captured image pairs. These inconsistencies contribute significantly to the limited cross-domain generalization performance of stereo matching networks. To overcome this challenge, we introduce a phase pre-normalization (PPN) method:
%彩色相位散斑赋予了场景额外的信息，然而相位信息淹没在投影到物体上的彩色散斑纹理中，对于不同场景中的物体，其颜色的反射率和光照条件均不一致，不同相机的ISP算法不一致也会导致拍摄到的数据产生域偏移，这些不一致是导致立体匹配网络跨域泛化性能受到限制的原因之一。因此，我们针对与物体表面反射率无关的相位信息进行归一化，提出了相位预归一化（PPN），具体原理为：
\begin{align}
    \varphi(x,y) &= \begin{aligned}[t]
    &\tan^{-1}\frac{2G(x,y)-R(x,y)-B(x,y)}{R(x,y)-B(x,y)} \\
    &= \tan^{-1}\frac{A(2g-b-r)+B\cos\varphi(2g+\frac{b}{2}+\frac{r}{2})}{A(r-b)+B\cos\varphi(\frac{r}{2}+\frac{b}{2})} \\
    &= \tan^{-1}\frac{B\cos\varphi(2g+\frac{b}{2}+\frac{r}{2})+w_1}{B\cos\varphi(\frac{r}{2}+\frac{b}{2})+w_2}
    \label{eq:norm}
    \end{aligned}
    \end{align}

Similar to the wrapped phase, the phase of deformed speckle is also constrained within \((- \pi, \pi)\). Equation \ref{eq:norm} indicates that, with an additional phase computation constraint, background light intensity is attenuated, while the active projection is amplified. Specifically, when the coefficients  \(r\), \(g\), \(b\) are nearly equal, the terms \(w_1\) and \(w_2\) become negligible, which means utilizing normalized phase as model input enhances feature distribution consistency across datasets. The pre-normalized phase is shown in Figure \ref{fig:norm}.
%与包裹相位相似，变形散斑的相位也在（-π, π）内被截断。由式(1)可知，在相位计算附加条件下，背景光强度被抑制，而我们的主动投影方式被增强。具体来说，当系数r、g、b接近时，wi、w2可以忽略。这意味着使用相位图作为模型的输入，即使在数据集之间，也可以增强特征分布的一致性。相位预归一化的过程如图5所示：

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{images/fig4_norm.png}
    \caption{In the scene of projected color speckle and the normalized image, it can be seen that the area projected speckle retains the phase information after pre-normalization, while the background area not projected speckle is ignored in this process.}
    \label{fig:norm}
\end{figure}

It can be observed that the phase information of the region within the green box, where speckle patterns are projected, is effectively preserved after pre-normalization. In contrast, the background region within the red box, which lacks projected colored speckles, has its texture information eliminated following pre-normalization. Consequently, in the image pairs input to the network, only the phase information from the object's surface is retained. This approach mitigates the adverse effects of ambient illumination and irrelevant background regions on the matching process. Moreover, the pre-normalization process leverages the Color Correction Matrix (CCM) characteristics of the color camera, ensuring that phase information is preserved in normally exposed images. This hardware-level consistency fundamentally guarantees domain uniformity, thereby alleviating issues related to inconsistent feature distributions across different scenes.
%可以看到，图中绿色框中被投影散斑的区域在经过预归一化之后的相位信息被充分保留，而红色框中的背景区域由于没有投影彩色散斑，在经过预归一化后的纹理信息被消除，这使得我们输入网络的图像对中，只有物体表面的相位信息被保留，从而避免了环境光照和不关心的背景区域对匹配产生负面影响，并且由于预归一化的原理利用了彩色相机的CCM矩阵特性，在正常曝光的图像上都能够保留相位信息，从硬件层面基本保证了域的一致性，从而避免了不同场景带来的特征分布不一致问题。
\subsection{RGB-Speckle Datasets}

Since existing public stereo datasets lack prior information, training the network on texture-based image pairs limits the ability to effectively learn phase features. Therefore, we employ an active binocular system to capture  complicated scenes projected by our RGB speckle patterns and the dense subpixel disparity ground truth by projecting Gray code patterns\cite{li2024three}. The scenes of our speckle datasets have abundant differences surface reflectance objects and repeated textures, which is very challenging for stereo matching. The illustration of our dataset is shown in Figure\ref{fig:dataset}.
%由于现有的双目公共数据集缺少彩色散斑所提供的额外相位信息，仅使用只有纹理信息进行训练限制了网络对相位特征的有效学习。为此，我们借助主动式双目系统，采用格雷码条纹得到稠密的视差groundtruth，并且投影了我们的彩色散斑图案。为了突出我们提出方法的有效性，我们在场景物体的表面反射率差异很大，光照环境复杂且存在大量病态区域的工业场景下采集数据集，这对于传统双目立体匹配是极具挑战的。数据集的示例如图6所示：

Though the ill-posed areas in these scenes are textured by speckles, it is difficult to obtain better results for the stereo matching network without the training of this kind of data. The reason is that the traditional method relies on color texture features, which shows poor generalization for scenes with huge differences in object surface reflectance, and the data of the network in other scenes will be affected by serious domain offset.
%从图6中可以看出，数据集中存在大量复杂场景，这些场景中的病态区域即使通过散斑赋予纹理，对于没有经过该类数据训练的立体匹配网络是难以得到较好效果的。原因是传统的方法依靠颜色纹理特征，对于物体表面反射率差异巨大的场景表现出极差的泛化性，网络在其他场景下的数据会受到严重的域偏移影响。

On the contrary, through the phase domain normalization and the phase information of the active projection, the model learns the matching relationship between the phase information independent of the reflectivity of the object surface, thus avoiding the domain offset problem, so that the model can still get better results in other scenarios.
%相反，通过相位域归一化以及主动投影的相位信息，模型学习到的是和物体表面反射率无关的相位信息之间的匹配关系，从而避免了域偏移问题，使得模型在其他场景下依旧能够得到较好的效果。

 By fine-tuning the stereo matching network with our phase pre-normalized speckle dataset,images captured by active binocular system that can project color speckles can reconstructed robustly even in previously unseen scenes. We anticipate that our provided speckle dataset will contribute to advancing the application and development of deep learning-based active binocular systems.
%对于任意能够投影彩色散斑的主动式双目系统，我们所采集的数据集同样适用，通过利用相位预归一化的散斑数据集对网络进行微调，就能在未见场景下得到优秀的重建效果。我们预期我们提供的散斑数据集能够为推动基于深度学习的主动式双目系统产品的应用和发展提供价值
\begin{figure} 
    \centering
    
    % 第一行，子图 (a)
    \begin{subfigure}[b]{0.45\linewidth} % 每张图宽度为页面宽度的45%
        \centering
        \includegraphics[width=\linewidth]{images/fig5a_origin.png} % 替换为你的图片文件名
        \caption{Origin scene}
        \label{fig:industrial scene}
    \end{subfigure}
    \hspace{2mm}
    % 第一行，子图 (b)
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/fig5b_graycode.png}
        \caption{Graycode}
        \label{fig:graycode}
    \end{subfigure}
    % 第二行，子图 (c)
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/fig5c_speckle.png}
        \caption{Speckle}
        \label{fig:subfig3}
    \end{subfigure}
    \hspace{2mm}
    % 第二行，子图 (d)
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/fig5d_gt.png}
        \caption{ Ground truth }
        \label{fig:subfig4}
    \end{subfigure}
    % 整个图的标题
    \caption{The production process of our speckle dataset. (a) A typical scene of our speckle dataset. (b)One of projected Gray code fringe. (c) Our projected color speckle. (d) The sub-pixel disparity ground truth.}
    \label{fig:dataset}
\end{figure}



==> sec_final/4_experiments.tex <==
\section{Experiments}

\begin{table*}
    \centering
    \begin{tabular}{cccc}
    \toprule
         Training & Validation & EPE & D1\\
    \midrule
        Scene Flow & Speckle (\textbf{PPN})& 21.406986 & 15.692858\\
        Scene Flow & Speckle & 15.853035 & 9.877504\\
        Scene Flow (\textbf{PPN}) & Speckle & 8.331100 & 5.238395\\
        Scene Flow (\textbf{PPN}) & Speckle (\textbf{PPN})& 5.120400 & 5.496406\\
        Speckle (\textbf{PPN}) & Speckle & 1.074344& 1.948889\\
        Speckle (\textbf{PPN}) & Speckle (\textbf{PPN})& \textbf{0.816987}& \textbf{1.105160}\\
    \bottomrule
    \end{tabular} 
    \caption{Comparison of ablation experiment  with EPE and D1}
    \label{tab:my_label} 
\end{table*}

\begin{figure*}
    \centering
    \includegraphics[width=0.85\linewidth]{images/fig6_Ablation.png}
    \caption{Accuracy performance across different training strategies. (a) Training on sceneflow and validation on phase pre-normalized(PPN) Speckle. (b) Training on sceneflow and validation on RGB Speckle. (c)Training on PPN sceneflow and validation on RGB Speckle. (d) Training on PPN sceneflow and validation on PPN Speckle. (e) Training on PPN Speckle and validation on RGB Speckle. (f) Training on PPN Speckle and validation on PPN Speckle. From top to bottom, the rows represent the input during the training phase, the input during the inference phase, and the error distribution within the mask. The bottom row shows the End-Point Error (EPE) of the computed disparity map.
    }
    \label{fig:scene_gt}
\end{figure*}

To validate the robustness of our approach, we conducted comprehensive quantitative and qualitative experiments. First, through ablation study, we analyzed the contribution of our phase-based method to the generalization performance of the network. Furthermore, we evaluated the robustness of our proposed method by comparing its performance across different stereo matching networks and various speckle patterns. Finally, we performed 3D reconstruction on unseen scenes to assess the method's cross-domain performance.
%为了验证我们方法的鲁棒性，我们进行了充分的定量及定性的实验，首先通过消融实验对比分析了我们的相位方法对网络泛化性能的提升。进一步，我们针对不同的立体匹配网络、不同的散斑图案对比验证了我们提出方法的鲁棒性。最后，我们针对未见场景进行三维重建，验证方法在跨域性能上的表现。

\subsection{Datasets and Metrics}
\paragraph{Datasets}To assess the performance of our proposed models and benchmark them against state-of-the-art methods, we evaluate the depth estimation accuracy using the SceneFlow dataset\cite{mayer2016large} and our custom RGB speckle dataset. The SceneFlow dataset, a widely recognized large-scale synthetic stereo matching benchmark, comprises 35,454 stereo image pairs for training and 4,370 pairs for testing, each with a resolution of 960$\times$540 pixels. Additionally, our RGB speckle dataset is designed to complement this evaluation by incorporating real-world speckle-patterned imagery, enabling a comprehensive analysis of depth estimation under distinct scene domains. And our speckle scene dataset contains 10716 image pairs and the resolution of the images is 1920$\times$1200 pixels acquired by an active binocular system. Given that our speckle dataset exhibits a significantly wider disparity range, we conducted training on the SceneFlow dataset at double the resolution to mitigate the risk of training instability or non-convergence caused by excessive disparities between the datasets.
%由于我们的散斑数据集视差范围较大，为了防止数据集之间视差范围差距过大引起的震荡不收敛，我们在sceneflow上的训练都是在两倍分辨率上进行的。

\paragraph{Metrics}Consistent with prior work in stereo matching, we adopt End-Point Error (\textbf{EPE}) and \textbf{D1} error rate as evaluation metrics to assess the performance of our proposed method. EPE is defined as the average absolute disparity error computed pixel-wise between the predicted disparity map and the corresponding ground truth. Meanwhile, the D1 error rate quantifies the fraction of pixels for which the absolute disparity error surpasses a specified threshold, such as 3 pixels.


\subsection{Implementation Details}

%In all experiments, we choose IGEV \cite{xu2023iterative} as our baseline, and we use the same strategy to train the model on sceneflow and speckle datasets. In the process of pre-training, we use the Sceneflow dataset with 1920*960 resolution. The purpose is to make the disparity range of the two data sets basically the same, so as to avoid the problem of unstable model training due to the large difference in disparity range during the training process. 
%在所有实验中，我们选择IGEV作为我们的baseline，采用pytorch和Adamw优化器实现，我们在sceneflow和speckle数据集上采用了相同的策略对模型进行了训练。在预训练的过程中，我们使用了2倍分辨率的Sceneflow数据集，目的是使训练的两个数据集视差范围基本一致，从而避免训练过程中由于视差范围差异过大导致模型训练不稳定的问题。

The experiments were conducted on four NVIDIA RTX 3090 GPUs. For the ablation study, we selected IGEV as the baseline model\cite{xu2023iterative}. The training process consisted of 140,000 iterations with a batch size of 12. Subsequently, we fine-tuned the model on our Speckle dataset for 350,000 iterations, employing a dataset split of 6:2:2 for training, validation, and testing, respectively. The initial learning rate was set to 0.0002, and training was performed using PyTorch with the AdamW optimizer, following the One-Cycle learning rate scheduling strategy. 
%The experiment was conducted on four NVIDIA 3090GPUs.我们以Batch size 为12训练了140,000个steps。随后以6:2:2的数据集划分方式在我们的散斑数据集上finetune了350,000个steps。设定初始学习率为0.0002，采用pytorch和Adamw优化器实现,并采用One-cycle学习率变化策略。

In stereo matching comparison experiments, we evaluate our approach against PSM-Net, ACV-Net, and RAFT-Stereo, three representative stereo matching networks\cite{chang2018pyramid,xu2022attention,lipson2021raftstereo}. Each network was trained to convergence on both the SceneFlow and Speckle datasets using PPN method.
%在立体匹配对比实验中，我们选择在PSM-Net，ACV-Net和RAFT-Stereo网络之间进行比较，各网络分别采用PPN策略在Sceneflow和Speckle数据集上训练至收敛。

We employed a binocular vision systems system consists of a color projector (XGIMI Z6X, resolution 1280$\times$720 pixels) paired with two cameras (Basler ace acA1920-40gc, resolution 1920$\times$1200 pixels, focal length 12 mm), featuring a baseline separation of 165 mm. The working distance for our system spans 0.5 to 1.5 meters.

\subsection{Ablation Study}

Since our method relies on an active binocular system to project additional speckle information onto objects, a direct comparison with prior approaches trained on public datasets would be inherently biased. Consequently, we designed our ablation studies to leverage both the SceneFlow and Speckle datasets. Specifically, we employed distinct training strategies on these datasets by incorporating phase pre-normalization selectively during training. The final evaluation was conducted exclusively on the validation set of our Speckle dataset, where we computed the End-Point Error (EPE) and D1 error rate to validate the enhancement of our method in improving the generalization performance of networks across diverse scenes.

To rigorously assess the effectiveness of our proposed method, we systematically partitioned the training and validation process into six controlled experimental groups. The performance of these groups is illustrated in Figure\ref{fig:scene_gt}:


%--------------------------消融实验描述-----------------------------
Firstly, We conducted inference on the speckle dataset using the weights pretrained on the SceneFlow dataset. The results indicate a markedly poor generalization performance, predominantly due to the network's dependence on color and texture features extracted directly from RGB images during the training process, especially on the speckle data after phase pre-normalization(PPN), where the significant domain gap renders the weights trained on RGB images entirely incompatible with phase maps, as illustrated in Figure\ref{fig:scene_gt} a. Moreover, a network trained solely on color and texture features exhibits domain sensitivity in scenes characterized by significant variations in object surface reflectance. Consequently, inference performance in other scenes is severely impacted by substantial domain shift, as demonstrated in Figure\ref{fig:scene_gt} b.
    %我们首先在sceneflow上预训练的IGEV权重对散斑数据集进行推理，可以看到表现出极差的泛化性，原因是直接通过RGB图像进行训练依靠颜色纹理特征，网络过度局部的纹理和底层的颜色信息，尤其是在经过PPN的散斑数据上，因为两者的域间距，在RGB图像上训练的权重对相位图完全不适用，如图6a所示。同时，仅利用色彩纹理训练的网络会对物体表面反射率差异巨大的场景下是域敏感的，在其他场景下的推理时会受到严重的域偏移影响，如图6b所示。

For the second training strategy, we apply Phase Pre-Normalization (PPN) to the SceneFlow dataset. Following network training on the PPN-processed iamge pairs, the accuracy on our speckle dataset exhibits greatly improvement. It demonstrate the effectiveness of our approach in enhancing cross-domain performance from synthetic to real datasets, as illustrated in Figure\ref{fig:scene_gt} c. Furthermore, when we inference on the speckle dataset after PPN, the network achieves higher accuracy, with notably lower error compared to the non-PPN-processed data, as shown in Figure Figure\ref{fig:scene_gt} d. This observation suggests that, even across datasets ranging from synthetic to real or from non-speckled to speckled domains, the normalized data domains remain closely aligned.
    %对于第二组，我们在sceneflow数据集上进行相位预归一化，网络在经过PPN后的数据训练后，极大提高了在我们散斑数据上的精度，这表明了我们的方法在Synthetic-to-Real数据集的跨域表现上是有效的，如图6c所示，并且，在对同样进行PPN的散斑数据集上推理时，网络表现出来的精度相对未经过PPN的误差更低如图6d所示，这表现出即使是合成到现实，无散斑到有散斑的数据集之间，归一化的数据域也是接近的。

Finally, we apply PPN on the speckle dataset and perform inference on both the original speckle images and PPN images respectively. The error is much lower than other group, as shown in \ref{fig:scene_gt}e and \ref{fig:scene_gt}f, and the best performance is achieved on the images after PPN, which fully illustrates the cross-scene capability of our proposed method.
    %对于第三组，我们在散斑数据集上进行相位预归一化，并分别在原始散斑图和预归一化之后的散斑图上进行验证，重建误差均远低于其他数据，如图6ef所示，并在经过PPN后的数据上取得了最好的表现，充分说明了我们所提出的方法的跨场景能力。

Table \ref{tab:my_label} shows the indicators calculated by our six training methods on the validation set of our speckle images. From the perspective of EPE and D1, the IGEV network trained with pre-normalization phase images has the best performance on the same PPN speckle validation images.Even in the speckle data without PPN, it can also have excellent performance. This result clearly demonstrates that a network trained on abundant normalized phase data effectively overcomes its reliance on color and texture features, enabling it to capture deeper phase-related features. Consequently, it delivers superior performance on images containing phase information without the need for pre-normalization, a capability that remains difficult to achieve across datasets devoid of phase information.
    %表1是我们的六种训练方式在散斑数据集的验证集上计算的指标,从EPE和D1上看，采用PPN的散斑数据进行训练的IGEV网络，在同样经过PPN的散斑验证集上的表现是最佳的，即使在未进行相位预归一化的散斑数据中也能拥有出色的表现，对于这一结果充分说明了经过预归一化后的网络，在拥有大量归一化后的散斑数据摆脱了对颜色纹理的依赖，从而学习到了更深层次的相位特征，在包含相位信息的图像即使不经过预归一化也能取得较好的效果，这在不含相位信息的数据集之间是难以实现的。
%-------------------------------------------------------------------


\begin{figure} % h 表示尽量放在当前位置
    \centering
    
    % 上面的子图 (a)
    \begin{subfigure}[b]{1\linewidth} % 宽度为页面宽度的80%，可以调整
        \centering
        \includegraphics[width=\linewidth]{images/fig7a_net.png} % 替换为你的图片文件名
        \caption{Scene 1}
        \label{fig:scene1}
    \end{subfigure}
    
    % 下面的子图 (b)
    \begin{subfigure}[b]{1\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/fig7b_net.png} % 替换为你的图片文件名
        \caption{Scene 2}
        \label{fig:scene2}
    \end{subfigure}
    
    % 整个图的标题
    \caption{The performance of different stereo matching networks under different projection speckle patterns.}
    \label{fig:net}
\end{figure}


%--------------------------不同网络对比实验描述-----------------------
Additionally, our approach imposes no constraints on the choice of stereo matching networks. The fundamental reason lies in the fact that we do not enhance cross-domain performance by modifying the network architecture itself; rather, we address this from the data perspective, improving the domain alignment of input data through preprocessing. To substantiate this, we trained PSM-Net, ACV-Net, and RAFT-Stereo on speckle data processed with PPN and conducted inference on two selected scenes from the speckle validation set with PPN, as illustrated in Figure\ref{fig:net}.
    %另外，我们的方法不限制立体匹配网络的选择，根本原因是我们并不是通过修改网络结构本身来提高网络的跨域性能，而是从数据本身出发，通过预处理来提高输入网络数据域的接近性，因此，我们也可以将相位预归一化的方法应用于其他立体匹配网络。为了验证这一点，我们在经过PPN后的散斑数据上对PSM-Net、ACV-Net和RAFT-Stereo进行训练，并且在验证集中选择了两个场景PPN后进行推理，如图7所示。

    As observed in the figure, these networks consistently achieve high-precision reconstruction results in regions containing phase information, underscoring the robustness of our approach. Additionally, we explored various permutations of speckle patterns disrupted in different ways across channels. The resulting new speckle patterns also yield favorable outcomes, attributable to the fact that phase information, modulated by the object, is embedded within a single image. Swapping this information across the three channels merely shifts the decoded phase values within the $(-\pi, \pi)$ interval without incurring any loss. Even when speckle patterns are processed through projection devices and the camera's Bayer filter, introducing phase deviations, the binocular system leverages redundant information to enhance robustness against noise, thereby minimizing adverse effects on disparity map reconstruction. Our method remains effective irrespective of system variations, provided the disparity range during training and inference remains consistent, rendering it applicable to other active binocular systems.
    %从图中可以看出，这些网络在包含相位信息的区域中均能够推理得到一致的高精度重建结果，说明了我们的方法的鲁棒性。另外，也对采用不同方式打乱的散斑进行通道间的排列组合，得到的新散斑图案同样能够取得较好的效果，这是由于经过物体调制后的相位信息嵌入在单张图片中，在三个通道中交换只会时解出的相位信息在（-Π，Π）区间中位置偏移，而不会有损失。即使散斑在经过投影设备和相机拜尔矩阵后，相位的偏差也会由于双目相机利用冗余的信息来换取系统对于噪声的鲁棒性而基本不对视差图的重建产生负面影响。因此我们的方法并不会由于系统的改变而失效，只要训练和推理的视差范围相同，就能适用于其他主动式双目系统。


%-------------------------------------------------------------------
%

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/fig8_unseen.pdf}
    \caption{Cross-scene performance display. The reconstruction details can be seen from the rightmost point cloud. }
    \label{fig:cross-scene}
\end{figure}

%--------------------------未见场景的对比实验描述-----------------------
The performance in unseen scenarios is our primary concern, as it directly determines whether our approach can be effectively applied to real-world 3D perception and precision measurement tasks. To rigorously evaluate generalization, we select scenarios that are entirely different from the synthetic and speckle data used for training. By projecting RGB speckle patterns and following our inference pipeline, we obtain the results shown in Figure \ref{fig:cross-scene}.
    %在未见场景中的表现是我们最关心的问题，因为这关系到我们的方法是否能够在实际的三维感知或者精度测量中应用。我们选择与训练的合成数据及散斑数据完全不一致的场景，通过投影RGB散斑，按照我们的流程进行推理后的结果如图8所示。

The figure presents various objects, including a monster model, two potted plants and a bucket. Our method demonstrates strong performance in these unseen scenarios. The reconstructed point cloud, derived from the disparity map, reveals that even in previously unseen regions—particularly along object boundaries—fine details are well preserved. This is attributed to the consistency of the phase information embedded in the speckle pattern across non-occluded areas. The experimental results validate the strong cross-scene generalization capability of our approach, offering a novel solution for active stereo systems.
    %图中展示了怪物模型，盆栽以及水桶等物体，我们的方法在这些未见场景中均取得了较好的效果，我们通过视差图重建得到的点云，可以看到对于未见区域，即使是在边缘区域也能重建出细节，这归功于散斑所蕴含的相位信息在未遮挡区域的表现是一致的。实验结果充分证明了我们的方法跨场景泛化能力，这对于主动式双目设备的应用提供了新方案。





%-------------------------------------------------------------------






==> sec_final/5_conclusion.tex <==
\section{Conclusion}
In this study, we proposed a novel RGB-Phase Speckle approach that introduces three key innovations: the generation of RGB color phase speckles, a phase pre-normalization technique, and a new speckle dataset tailored for stereo matching tasks. Our method effectively addresses the significant reliance of deep learning-based active binocular systems on data consistency by leveraging phase pre-normalization, which aligns data domains and enhances model generalization. This advancement facilitates the practical deployment of active binocular systems in diverse real-world scenarios. Experimental results demonstrate that our method achieves accurate and robust depth inference across images captured by physical systems with identical configurations, irrespective of the scene. This improved generalization highlights the potential of our approach in challenging environments where traditional methods struggle.
%我们提出了rgb散斑，主要贡献包含了RGB彩色散斑，相位预归一化，以及按照所提出方法得到的彩色散斑数据集，我们的方案不限制立体匹配网络的选择，借助单个彩色散斑数据集训练的网络权重可以用于采用相同结构搭建的物理系统在任意场景下得到的图像进行准确的深度推理，从硬件系统层面克服了目前基于深度学习的主动式双目系统对数据一致性的严重依赖，借助相位预归一化，我们推动解决了跨场景泛化性的问题，摆脱了针对不同场景使得主动式双目系统实现单帧动态场景稠密感知甚至三维测量（脱离实验室），真正应用于实际场景成为了可能。

Future research will focus on optimizing projection hardware to achieve reduced costs, smaller form factors, faster projection speeds, and improved energy efficiency. Additionally, we aim to further explore the miniaturization, integration, and generalization of active binocular systems to expand their practical applicability in real-world measurement tasks.


%未来工作的探索将针对投影的设备进行优化，使得散斑投影设备能够实现更低的成本，更小的体积，更快的投影速度，以及更低的能耗，对主动式双目系统进行小型化，集成化和通用化进行进一步的研究。


